Necessary and sufficient condition for a generic 3R serial manipulator to be cuspidal

Cuspidal robots can travel from one inverse kinematic solution to another without meeting a singularity. The name cuspidal was coined based on the existence of a cusp point in the workspace of 3R serial robots. The existence of a cusp point was proved to be a necessary and sufficient condition for orthogonal robots to be cuspidal, but it was not possible to extend this condition to non-orthogonal robots. The goal of this paper is to prove that this condition stands for any generic 3R robot. This result would give the designer more flexibility. In the presented work, the geometrical interpretation of the inverse kinematics of 3R robots is revisited and important observations on the nonsingular change of posture are noted. The paper presents a theorem regarding the existence of reduced aspects in any generic 3R serial robot. Based on these observations and on this theorem, we prove that the existence of a cusp point is a necessary and sufficient condition for any 3R generic robot to be cuspidal.

==> abbreviations.tex <==
%%%%%%%%%%% declare: abbreviations %%%%%%%%%%%
\abbrev{degrees of freedom}{dof}
\abbrev{inverse geometric solution}{IGS}
\abbrev{direct geometric solution}{DGS}
\abbrev{direct geometric model}{DGM}
\abbrev{Denavit Hartenberg}{DH}
\abbrev{centre of rotation}{COR}
\abbrev{end-effector}{EE}
\abbrev{collision free workspace}{CFW}
\abbrev{forward instantaneous kinematic problem}{FIKP}
\abbrev{inverse instantaneous kinematic problem}{IIKP}
\abbrev{Universal joint}{U}
\abbrev{Spherical joint}{S}
\abbrev{Spherical Parallel Mechanism}{SPM}
\abbrev{Rotational joint}{R}
\abbrev{Genetic Algorithm}{GA}
\abbrev{Nelder-Mead}{NM}
\abbrev{Operating Room}{OR}
\abbrev{Centre Hospitalier Universitaire}{CHU}
\abbrev{Parallel Kinematic Manipulator}{PKM}
\abbrev{Non-dominated Sorting Genetic Algorithm}{NSGA-II}
\abbrev{Multi-Objective Evolutionary Algorithm based on Decomposition}{MOEA/D}
\abbrev{Particle Swarm Optimization}{PSO}
\abbrev{Multi Objective Optimization}{MOO}
\abbrev{Differential Evolution}{DE}
\abbrev{Regular Dextrous Workspace}{RDW}
\abbrev{Spherical-Spherical}{SS}
\abbrev{Universal-Spherical}{US}
\abbrev{Revolute-Revolute}{RR}

\DeclareAcronym{CAD_model}{
  short = CAD modeling,
  long  = Computer Aided Design,
  class = abbreviations
}

==> notations.tex <==
%%%%%%%%%%% declare: notations %%%%%%%%%%%
\notat{generalized output vector}{op_vec}{$\mathbf{x}$}
\notat{input vector}{ip_vec}{$\mathbf{q_i}$}
\notat{slack/surplus variable vector}{var_vec}{$\mathbf{s}$}
\notat{configuration space}{c_space}{$\mathcal{D}$}
\notat{input space}{ip_space}{$\mathcal{I}$}
\notat{output space}{op_space}{$\mathcal{K}$}
\notat{optimisation space}{o_space}{$\mathcal{O}$}
\notat{special Euclidean group of dimension 3}{se3}{\textit{SE}(3)}
\notat{special orthogonal group of dimension 3}{so3}{\textit{SO}(3)}
\notat{pose of the mechanism}{pose}{$\mathbf{x}$}
\notat{actuation joint vector}{act_q}{$\mathbf{q}_a$}
\notat{output twists}{op_twist}{$\mathbf{t}$}
\notat{feasible set}{FS}{$\mathcal{F}$}
\notat{quality index}{qi}{$\kappa^{-1}$}
\notat{manipulability ellipsoid volume}{ev}{$v_e$}
\notat{conditioning number}{cnum}{$\kappa$}
\notat{Jacobian matrix}{jac}{$\mathbf{J}$}
\notat{global quality index}{gqi}{$\kappa^{-1}_{g}$}
\notat{desired Regular Dextrous Workspace}{dRDW}{RDW$_d$}
